Matching 2D Images in 3D: Metric Relative Pose from Metric Correspondences

Given two images, we can estimate the relative camera pose between them by establishing image-to-image correspondences. Usually, correspondences are 2D-to-2D and the pose we estimate is defined only up to scale. Some applications, aiming at instant augmented reality anywhere, require scale-metric pose estimates, and hence, they rely on external depth estimators to recover the scale. We present MicKey, a keypoint matching pipeline that is able to predict metric correspondences in 3D camera space. By learning to match 3D coordinates across images, we are able to infer the metric relative pose without depth measurements. Depth measurements are also not required for training, nor are scene reconstructions or image overlap information. MicKey is supervised only by pairs of images and their relative poses. MicKey achieves state-of-the-art performance on the Map-Free Relocalisation benchmark while requiring less supervision than competing approaches.

==> rebuttal/easy_vs_hard_example.tex <==
\begin{figure}[t]
  \centering
   \includegraphics[width=1.0\linewidth]{rebuttal/images/visual_vs_non_examples_v5.pdf}
   \vspace{-1.4em}
   \caption{
   \ours finds visual corresponding matches in overlapping images, but also reasons about the image to propose matches beyond local patterns under extreme viewpoint changes.
   % , \eg, opposing view pairs. 
   % is able to solve image pair with easy and extreme viewpoint changes, \eg, opposing view pairs. 
   % \ours relies on low-level patterns where there is visual overlap, but finds establishes correspondences for the AR task when 
   % and reasons about the image, \eg, the shape of the statue, is able to find accurate keypoint correspondences when there is visual overlap, however, when there is no visual overlap, \ours provides matches beyond local structures, allowing to compute valid relative poses for pairs that were unsolvable until now.
   }
   \label{reb:fig:easy_vs_hard}
\end{figure}

% \begin{figure}[t]
%   \centering
%    \includegraphics[width=1.0\linewidth]{rebuttal/images/visual_vs_non_examples_v2.pdf}
%    \caption{
%    \ours estimates visual corresponding matches in overlapping images, but also reasons about the image to propose matches beyond local patterns under extreme viewpoint changes.
%    \axel{Hard example already in Supplementary material}.
%    % , \eg, opposing view pairs. 
%    % is able to solve image pair with easy and extreme viewpoint changes, \eg, opposing view pairs. 
%    % \ours relies on low-level patterns where there is visual overlap, but finds establishes correspondences for the AR task when 
%    % and reasons about the image, \eg, the shape of the statue, is able to find accurate keypoint correspondences when there is visual overlap, however, when there is no visual overlap, \ours provides matches beyond local structures, allowing to compute valid relative poses for pairs that were unsolvable until now.
%    }
%    \label{reb:fig:easy_vs_hard}
% \end{figure}

% \begin{figure}[t]
%   \centering
%    \includegraphics[width=1.0\linewidth]{rebuttal/images/visual_vs_non_examples_v3.pdf}
%    \caption{
%    \ours estimates visual corresponding matches in overlapping images, but also reasons about the image to propose matches beyond local patterns under extreme viewpoint changes.
%    % , \eg, opposing view pairs. 
%    % is able to solve image pair with easy and extreme viewpoint changes, \eg, opposing view pairs. 
%    % \ours relies on low-level patterns where there is visual overlap, but finds establishes correspondences for the AR task when 
%    % and reasons about the image, \eg, the shape of the statue, is able to find accurate keypoint correspondences when there is visual overlap, however, when there is no visual overlap, \ours provides matches beyond local structures, allowing to compute valid relative poses for pairs that were unsolvable until now.
%    }
%    \label{reb:fig:easy_vs_hard2}
% \end{figure}

==> sec/3_method_old.tex <==
\input{figures/system_fig}
\section{Method}
\label{sec:method}
In this section, we explain how we compute the metric relative pose $T = (R, t)$ given \textit{I} and \textit{I'} input images.
We first start defining the architecture and then the main components of our differentiable pose solver. Figure \ref{fig:system} shows our full pipeline.

%%------------   Architecture   ------------
\subsection{Architecture}
\label{sec:method:arch}
\input{figures/architecture_fig}
\ours follows a multi-head network architecture with a shared encoder \cite{tyszkiewicz2020disk, revaud2019r2d2, detone2018superpoint} that infers 3D metric keypoints and descriptors from an input image.
\smalljump

\noindent\textbf{Encoder.} We adopt a pre-trained DINOv2 as our feature extractor \cite{oquab2023dinov2}, and use its features without further training or fine-tuning. DINOv2 divides the input image into $14 \times 14$ patches and provides a feature vector for each position, resulting in an output feature map $F$, of resolution $(1024, w, h)$, where $w=W/14$ and $h=H/14$.
\smalljump

\noindent\textbf{Keypoint Heads.} 
We define four parallel heads that process the feature map $F$ to generate the \textit{xy} offset ($U^{2\times w\times h}$), depth ($Z^{w\times h}$), confidence ($C^{w\times h}$), and descriptor ($D^{128\times w\times h}$) maps; where each entry of those maps corresponds to a $14 \times 14$ patch in the input image. 
Similar to \cite{christiansen2019unsuperpoint}, \ours has the rare property of predicting keypoints as relative offsets to a sparse regular grid. Thus, contrary to methods that rely on a dense heat map based on filter responses \cite{lenc2016learning, verdie2015tilde, barroso2019key}, \ours allows for high level reasoning. We obtain the absolute 2D keypoint coordinates ($\bar{U}$) as: 
% by adding the predicted offset to its row/column position and then multiplying them by the downsampling factor $f=14$:
\begin{equation}
\begin{gathered}
    \bar{u}_{ij} = f * [u_i + i, u_j + j], \text{with } \xspace U \in [0, 1],
\label{eq:abs_coordinates}
\end{gathered}
\end{equation}
where \textit{f} refers to the encoder downsampling factor ($f=14$) and $ij$ to its grid position. 
% We then can lift keypoints to camera coordinates by combining the $\bar{C}$ 2D locations and \textit{Z} depth values together with the camera intrinsics \textit{K} as $X_{ij} = Z_{ij} K^{-1} \bar{C_{ij}}$. For simplicity, we ifnore homogenoeus coordinates.  
The architecture remains efficient due to its sparsity but still provides correspondences at sub-pixel level. 
We show the architecture in Figure \ref{fig:architecture}.

%------------   Learning from Metric Pose Supervision   ------------
\subsection{Learning from Metric Pose Supervision}
We aim at training our relative pose estimation method in an end-to-end fashion. Meaning that, we want to directly optimize the parameters of our network to produce accurate relative poses. During training, we assume to have training data as ($I$, $I'$, $T^{GT}$, $K$, $K'$), with $T^{GT}$ being the ground truth transformation and $K/K'$ the camera intrinsics. 

To learn 3D keypoint coordinates, confidences and descriptors, we require our system to be fully differentiable, and since some of the elements of the pipeline are not, \eg, keypoint sampling or inlier counting, we redefine the relative pose estimation pipeline as probabilistic.

\subsubsection{Probabilistic Correspondence Selection}
\label{sec:method:sampling}
We first establish how we sample a set of keypoint correspondences, $\mathcal{Y}$, given the outputs of the network.
\smalljump

\noindent\textbf{Matching Distribution.}
Given the descriptors maps, \textit{D} and \textit{D'}, we compute the cosine similarity between the descriptors to obtain the similarity matrix $m^{(w \times h) \times (w' \times h')}$. Following \cite{tyszkiewicz2020disk, sun2021loftr, edstedt2023dedode}, we enforce a soft cycle-consistency matching through a dual-Softmax operator, where we first compute the probability of descriptors \textit{D} matching \textit{D'} ($P_{D \rightarrow D'}$), and multiply it with its reverse ($P_{D \leftarrow D'}$). Thus, the probability of two descriptor $d_i$ and $d'_j$ being nearest neighbours of each other is defined as:
\begin{equation}
\begin{gathered}
    M_{I \leftrightarrow I'}(i \leftrightarrow j) = P_{D \rightarrow D'}(i\vert m, j) \cdot P_{D \leftarrow D'}(j\vert m, i), \\
    \text{and} \quad P_{D \rightarrow D'}(i\vert m, j) = \text{Softmax}(m(i, \cdot)/\theta_m)_j,
\end{gathered}
\label{eq:desc_softmax}
\end{equation}
\begin{equation}
\begin{gathered}
    P_{I \leftrightarrow I'}(i, j) = P_{I \leftarrow I'}(j\vert i) \cdot P_{I}(i) \cdot P_{I \rightarrow I'}(i\vert j) \cdot P_{I'}(j) , \\
    \text{and} \quad P_{I \rightarrow I'}(i\vert j ; m) = \text{Softmax}(m(i, \cdot)/\theta_m)_j,
\end{gathered}
\label{eq:desc_softmax_alt}
\end{equation}
where $\theta_m$ is the descriptor Softmax temperature. Before the normalization, we augment $m$ with a single learnable dustbin parameter to allow unmatched keypoints to be assigned to it \cite{sarlin2020superglue}. We remove the dustbin after the dual-Softmax layer.
\smalljump

\noindent\textbf{Keypoint Distribution.}
We treat the score confidence maps, $C$ and $C'$, as a probability distribution over the keypoint locations. For that, we apply a spatial Softmax operator to normalize the maps independently, where each position in a map represents how likely a keypoint is to generate a good pose. Similar to the descriptor matrix, we combine $C$ and $C'$ into a single keypoint probability matrix 
% $N_{I \leftrightarrow I'}^{(w \times h) \times (w' \times h')}$
$N_{I \leftrightarrow I'}$, where each entry represents the probability of selecting two independent keypoints from \textit{I} and \textit{I'}. 
Note that instead of applying a local non-maxima suppression \cite{tyszkiewicz2020disk, barroso2020hdd, luo2020aslfeat}, \ours already provides a single keypoint location for every input patch.
\smalljump

\noindent\textbf{Correspondence Selection.}
The total probability of sampling a keypoint correspondence is modelled as a function of their descriptor similarities ($M_{I \leftrightarrow I'}$) and the keypoint selection probabilities ($N_{I \leftrightarrow I'}$). Thus, the probability of selecting keypoint $i$ and $j$ from \textit{I} and \textit{I'} as a correspondence is: 
\begin{equation}
\begin{gathered}
    P_{I \leftrightarrow I'}(i, j) = M_{I \leftrightarrow I'}(i, j) \cdot N_{I \leftrightarrow I'}(i, j).
\label{eq:corr_selection}
\end{gathered}
\end{equation}
This distribution assigns a high probability to correspondences that have similar and discriminative descriptors and at the same time belong to repeatable and accurate locations, while assigns low probabilities in all other cases, \eg, sky regions where there are similar descriptors but are not unique. 
We finally sample a complete set of \textit{Y} correspondences $\mathcal{Y} = \{y_{i}\}$ according to $P_{I \leftrightarrow I'}$. 

\subsubsection{Differentiable RANSAC}
Due to the probabilistic nature of our approach and potential errors in our network predictions, we rely on the robust estimator RANSAC \cite{fischler1981random} to compute pose hypotheses $h$ from $\mathcal{Y}$. We require our RANSAC layer to backpropagate the pose error to the keypoints and descriptors, and hence, we follow differentiable RANSAC works \cite{bhowmik2020reinforced, brachmann2021visual, brachmann2019neural}, and adjust them as necessary for our problem:
\smalljump

\noindent\textbf{Generate hypotheses.} Given the set of $\mathcal{Y}$ correspondences, we use its $P_{I \leftrightarrow I'}$ values to guide the new sampling of $J$ subsets $\mathcal{J}_j \subset \mathcal{Y}$, with $0 \leq j < J-1$. Every subset is defined by \textit{n} 3D-3D correspondences in camera coordinates, where the relationship of a 3D point $x_i$ and its 2D coordinates ($\bar{u}_i$) and depth ($z_i$) is: 
\begin{equation}
\begin{gathered}
    x_i = z_i \cdot K^{-1} \bar{u}_i^T.
\label{eq:camera_coor}
\end{gathered}
\end{equation}
$K$ refers to the camera intrinsics, and for notation simplicity, we assume homogeneous coordinates for 2D points ($\bar{u}$). Each correspondence subset $\mathcal{J}_j$ generates a pose hypothesis $h_j$, which we compute using a pose solver $g$, \ie, $h_j=g(\mathcal{J}_j)$.
\smalljump

\noindent\textbf{Soft-Inlier Counting.} Since counting inliers is not differentiable, we compute a differentiable approximation of the inlier counting (soft-inlier counting) by replacing the hard threshold by a Sigmoid function $\sigma(\cdot)$:
\begin{equation}
\begin{gathered}
    s(h, \mathcal{Y}) = \sum_{y_i \in \mathcal{Y}} \sigma [\beta \tau - \beta r(y_i, h)].
\end{gathered}
\label{eq:softInlier}
\end{equation}
$r(\cdot)$ refers to the error function, and the hyper-parameter $\beta$ controls the softness of the Sigmoid. As in \cite{brachmann2021visual}, we define the heuristic in dependence of the inlier threshold $\tau$ such that $\beta=\frac{5}{\tau}$.
\smalljump

\noindent\textbf{Differentiable Refinement.} We refine the pose hypothesis $h$ by iteratively finding its correspondence inliers $\mathcal{I}$ and recomputing a new pose from them:
\begin{equation}
\begin{gathered}
    h^{t+1} = g(\mathcal{I}^t) \quad  \text{and} \quad \mathcal{I}^{t+1} = \{i \vert r(y_i, h^{t+1}) < \tau\}.
\end{gathered}
\end{equation}

We repeat the process until a maximum number of iterations $t_\text{max}$ is reached, or the number of inliers stops growing. We then approximate the gradients of the refinement step by fixing and backpropagating only through its last iteration.
\smalljump

\noindent\textbf{Differentiable Solver.}
We use the Kabsch pose solver \cite{kabsch1976solution} for estimating the metric relative pose from the 3D-3D correspondences. We obtain 3D keypoints from network outputs (as seen in Equation \ref{eq:camera_coor}) and correspondences ($\mathcal{Y}$) as explained in Section \ref{sec:method:sampling}. We apply the same solver to the initial sets ($\mathcal{J}_j$) or during pose refinement ($\mathcal{I}$). The Kabsch solver finds the pose that minimizes the square residual over the subset of correspondences: 
\begin{equation}
\begin{gathered}
g^{\text{Kabsch}}(\mathcal{J}) = \argminB_{h} \sum_{y_i \in \mathcal{J}} r(y_i, h)^2.
\end{gathered}
\end{equation}
The residual error function $r(\cdot)$ computes the euclidean distance between 3D keypoint correspondences after applying the pose transformation $h$. All the steps within the Kabsch solver are differentiable and have been previously studied, and hence, we refer to \cite{brachmann2021visual, avetisyan2019end} for additional details.

\subsubsection{Learning Objective}
\label{sec:method:loss}
We use the Virtual Correspondence Reprojection Error (VCRE) metric proposed in \cite{arnold2022map} as our loss function. VCRE defines a set of virtual points in homogeneous coordinates $\mathcal{V}$ and computes the euclidean error of its projections in the image:
\begin{equation}
\begin{gathered}
\ell^{\text{VCRE}}(h, \hat{h}) =\frac{1}{\vert\mathcal{V}\vert} \sum_{v \in \mathcal{V}}\vert\vert\pi(v) - \pi(h\hat{h}^{-1}v)\vert\vert_2,
\label{eq:vcre}
\end{gathered}
\end{equation}
with $\hat{h}=T^{GT}$ and $\pi$ being the projection function. Refer to supplementary details for more details on VCRE.  
As mentioned, for each $\mathcal{Y}$, we compute a set of hypotheses $h_j$ and their corresponding scores $s_j$. We approximate its expected loss by applying a Softmax over $s_j$ and use the normalized scores ($\bar{s}_j$) to aggregate each hypothesis loss as: 
\begin{equation}
\begin{gathered}
\ell({\mathcal{Y}}, \hat{h}) \approx \sum_{j \in J} \bar{s}_j \ell^{\text{VCRE}}(R(h_j, \mathcal{Y}), \hat{h}), \text{where} \\
\ell({\mathcal{Y}}, \hat{h}) = \E_{j  \sim p(j \vert \mathcal{Y})} [s_j \cdot \ell^{\text{VCRE}}(R(h_j, \mathcal{Y}), \hat{h})].
\label{eq:loss_Y}
\end{gathered}
\end{equation}
We assign a single loss value to $\mathcal{Y}$ to ensure that our RANSAC is robust to some degree of noise and learns to assign low scores to poses with high errors. 
We then define our final optimization as the expectation of the VCRE loss \wrt sampling correspondence sets $\mathcal{Y}_k$ from the correspondence matrix $P_{I \leftrightarrow I'}$:
\begin{equation}
\begin{gathered}
\mathcal{L}(P_{I \leftrightarrow I'}, \hat{h}) = \E_{k  \sim p(k \vert P_{I \leftrightarrow I'})} [\ell({\mathcal{Y}_k}, \hat{h})].
\end{gathered}
\end{equation}
From now on, we abbreviate $\mathcal{L}(P_{I \leftrightarrow I'}, \hat{h})$ to $\mathcal{L}$ and $\ell({\mathcal{Y}_k}, \hat{h})$ to $\ell$. We can approximate $\mathcal{L}$ gradients by drawing $K$ samples \wrt to network parameters ($w_1, w_2 \subset w$): 
\begin{equation}
\begin{gathered}
\frac{\partial}{\partial w} \mathcal{L} \approx \frac{1}{K} \sum_{k \in K} [\ell \frac{\partial}{\partial w_1} \text{log} P_{I \leftrightarrow I'} + \frac{\partial}{\partial w_2}\ell],
\end{gathered}
\end{equation}
\axel{Is using $w_1$ and $w_2$ ok? Or should we just use $w$?}
where $w_1$ refers to descriptor and keypoint confidence head parameters, while, $w_2$ refers to the keypoint offset and depth heads. Note that the first term ($w_1$) only provides a signal steering the sampling probability $P_{I \leftrightarrow I'}$ in a good direction, and thus, we rely on REINFORCE algorithm \cite{williams1992simple} to reduce the variance by subtracting a baseline ($b = \E_k[\ell]$ \axel{or $b=\bar{\ell}$?}) from $\ell$:
\begin{equation}
\begin{gathered}
\frac{\partial}{\partial w} \mathcal{L} \approx \frac{1}{K} \sum_{k \in K} [[\ell-b] \frac{\partial}{\partial w_1} \text{log} P_{I \leftrightarrow I'} + \frac{\partial}{\partial w_2}\ell].
\end{gathered}
\end{equation}
\axel{Add more observations? They could go into Supp.}

\subsubsection{Curriculum Learning}
\label{sec:curr_learning}
Initialization is an important and challenging step when learning only from poses \cite{bhowmik2020reinforced}. 
One common solution in RL is to feed the network with increasingly harder examples that may otherwise be too difficult to learn from scratch \cite{narvekar2020curriculum}.
However, contrary to other methods \cite{sarlin2020superglue, sun2021loftr, edstedt2023roma}, we aim at training our network without requiring to know what \textit{easy} or \textit{hard} examples are. 
Assuming a batch $B$, we define the hardest example as the image pair with the highest loss. Instead of using the full batch $B$ in our training, we optimize the network only using a small subset of image pairs. We select the subset of image pairs that return the lowest losses, \ie, network is optimized only with the examples that can solve better, and hence, are \textit{easier}.
As we progress in the training, we use more examples from $B$. We define both, the minimum and maximum number of pairs ($b_{\text{min}}$ and $b_{\text{max}}$), used in training.  
Even though we limit the optimization to the best pose estimates, in some cases, the network tries to optimize image pairs where all hypotheses are incorrect, misleading the overall objective and adding noise to the gradients of good poses. 
To mitigate this, we add a \textit{null hypothesis} ($h^0$) to Equation \ref{eq:loss_Y}. 
We assign a weight $s^0$ and determine its loss as $\ell^{\text{VCRE}}(h^0)=\text{VCRE}^{\text{max}}$, where $\text{VCRE}^\text{max}$ is the maximum value we tolerate as a \textit{good} pose. $h^0$ serves as an anchor point, such that the network can assign lower scores than $s^0$ to those hypotheses with higher error than $\text{VCRE}^\text{max}$. This serves as a mechanism to reduce the magnitude of the misleading gradients that go into the network. 
% This simple yet effective strategy allows training \ours from scratch without further supervision than the poses. 

